Active Learning for Coreference Resolution using Discrete Annotation

We improve upon pairwise annotation for active learning in coreference resolution, by asking annotators to identify mention antecedents if a presented mention pair is deemed not coreferent. This simple modification, when combined with a novel mention clustering algorithm for selecting which examples to label, is much more efficient in terms of the performance obtained per annotation budget. In experiments with existing benchmark coreference datasets, we show that the signal from this additional question leads to significant performance gains per human-annotation hour. Future work can use our annotation protocol to effectively develop coreference models for new domains. Our code is publicly available at https://github.com/belindal/discrete-active-learning-coref .

==> 06_discussion.tex <==


We conduct analyses into the type of examples our model captures


% Mention something about how applicable this collected dataset is to other models
Since active learning generally functions on top of a single underlying model, it is unclear whether labels collected through active learning can be more beneficial for other models. We leave this exploration to future work. Regardless, we propose our discrete annotation \textit{approach} as a cost-effective method for collecting coreference annotations, which can be used in either active learning or more general annotation settings.


